Cortex: A Compiler for Recursive Deep Learning Models

Optimizing deep learning models is generally performed in two steps: (i) high-level graph optimizations such as kernel fusion and (ii) low level kernel optimizations such as those found in vendor libraries. This approach often leaves significant performance on the table, especially for the case of recursive deep learning models. In this paper, we present Cortex, a compiler-based approach to generate highly-efficient code for recursive models for low latency inference. Our compiler approach and low reliance on vendor libraries enables us to perform end-to-end optimizations, leading to up to 14X lower inference latencies over past work, across different backends.

==> src/backend_summary_table.tex <==
DyNet  & 9.17 & 4.31 & 3.08\\


==> src/cavs_table.tex <==
$h_s$ & 1 & 0.97/\textbf{0.09} & 10.24 & 1.95/\textbf{0.15} & 12.94 & 2.54/\textbf{0.22} & 11.38 \\
$h_s$ & 10 & 3.74/\textbf{0.27} & 14.06 & 3.28/\textbf{0.27} & 12.18 & 4.01/\textbf{0.44} & 9.05 \\
$h_l$ & 1 & 1.22/\textbf{0.16} & 7.41 & 2.01/\textbf{0.2} & 10.22 & 2.56/\textbf{0.28} & 9.04 \\
$h_l$ & 10 & 5.8/\textbf{0.69} & 8.46 & 3.66/\textbf{0.61} & 5.96 & 4.43/\textbf{0.91} & 4.88 \\


==> src/design.tex <==
\section{Design}\label{sec:design}
In this section, we discuss each component of the pipeline in
detail. First, we give some background on tensor compilers
(\S\ref{sec:tensor_comp}), then describe the Recursive API
(\S\ref{sec:rec_api}) and the ILIR (\S\ref{sec:ilir_api}), and then
move on to the compiler lowering passes (\S\ref{sec:rec_lower} and
\S\ref{sec:ilir_lower}).

\subsection{Tensor Compilers}\label{sec:tensor_comp}
\Sys's interface is influenced by past work on tensor compilers. A
tensor compiler allows users to express tensor computations and
generate optimized code for them. In most tensor compilers,
computation and optimizations are specified separately. The tensor
computation is expressed as a DAG (directed acyclic graph) of
operators, each of which produce a tensor by consuming previously
produced or input tensors. After expressing the computation, the user
can use scheduling primitives to perform optimizations such as tiling,
unrolling, vectorization, etc. Fig.~\ref{fig:tensor_comp_eg} shows how
elementwise matrix addition may be expressed and optimized in a tensor
compiler.

\begin{figure}
  \includegraphics[width=1.0\linewidth]{fig/tensor_compiler_eg}
  \caption{Elementwise matrix addition in a tensor compiler}
  \label{fig:tensor_comp_eg}
\end{figure}

\subsection{Recursive API (RA)}\label{sec:rec_api}
This API allows the user to express models that involve recursive
computations over data structures along with dense tensor
algebra. Along with the higher level recursive control flow, the input
program needs to contain enough information about the tensor
operations performed in the model to enable scheduling when it is
lowered to ILIR (\textbf{C.2} in Fig.~\ref{fig:pipeline}).
Accordingly, the RA models an input computation as a DAG of operators
where each operator is specified as a loop nest. This is seen in
Listing~\ref{code:treernn_ra} which shows the simplified model from
Fig.~\ref{fig:treelstm} as expressed in RA.

%% Accordingly, the RA models an input computation as a DAG of
%% operations, much like the dataflow graph in TensorFlow, where each
%% operator is specified as a loop nest, much like in a tensor
%% compiler. This is seen in Listing~\ref{code:treernn_ra} which shows
%% the simplified model from Fig.~\ref{fig:treelstm} as expressed in RA.

\begin{listing}[h]
\begin{minted}[escapeinside=||,linenos,numbersep=4pt,frame=lines,fontsize=\scriptsize]{src/ra_lexer.py:RALexer -x}
################## Model computation ##################
# H: Hidden and embedding size
# V: Vocabulary size
# N: Total number of nodes in the input data structure(s)
Tensor Emb = input_tensor((V,H))
Tensor word = input_tensor((N))

# A placeholder that represents results of recursive calls
Tensor rnn_ph = placeholder((N,H))
# Base case definition
Tensor leaf_case =
  compute((N,H), lambda n,i: Emb[word[n],i])
# Recursive body definition
Tensor lh = compute((N,H), lambda n,i: rnn_ph[n.left,i])
Tensor rh = compute((N,H), lambda n,i: rnn_ph[n.right,i])
Tensor recursive_case =
  compute((N,H), lambda n,i: tanh(lh[n, i]+rh[n, i]))
# Conditional check for the base case
Tensor body = if_then_else((N,H), lambda n,i: isleaf(n),
                           leaf_case, recursive_case)
# Finally, create the recursion
Tensor rnn = recursion_op(rnn_ph, body)

############### RA scheduling primitives ###############
dynamic_batch(rnn)                                                |\label{line:ra_sched1}|
specialize_if_else(body)                                          |\label{line:ra_sched2}|
\end{minted}
\captionof{listing}{Model in Fig.~\ref{fig:treelstm} as expressed in
  the RA.}
\label{code:treernn_ra}
\end{listing}

We observe that recursive deep learning model computations often
satisfy the following properties:

\begin{enumerate}[label=\textbf{P.\arabic*}, leftmargin=2em]
\itemsep0em
\item \label{prop:ds_ctrl} All control flow depends on the
  connectivity of the data structure, and not on dynamically computed
  data.
\item \label{prop:first_call} All recursive calls can be made before
  performing any tensor computation.
\item \label{prop:ind_calls} Recursive calls to the children of a data
  structure node are independent of each other i.e.~the arguments to
  one call do not depend on the results of a previous call.
\end{enumerate}

Property~\ref{prop:ds_ctrl} implies that we know all the control flow
during the model execution before the execution in the form of the
data structure. Property~\ref{prop:first_call} entails that the
computation starts at the leaves of the data structure, moving up
towards the roots, while property~\ref{prop:ind_calls} means that
sibling nodes can be processed in parallel, which enables us to
perform dynamic batching more effectively. The RA and later
compilation stages exploit these properties of the input models.

While not shown in Listing~\ref{code:treernn_ra}, the user needs to
provide basic information about the input data structure such as the
maximum number of children per node, and the kind of the data
structure (sequence, tree or DAG). This information is used during
compilation, and can be easily verified at runtime.

\subsubsection{Recursion Scheduling Primitives}\label{sec:rec_sched}
When lowering the recursive computation to loops, we need to ensure
that the data dependences between the data structure nodes are
satisfied. However, as these dependences generally specify only a
partial ordering on the nodes, we have significant freedom when
scheduling the computations. Different schedules may afford different
degrees of parallelism, or allow for data
reuse. Lines~\ref{line:ra_sched1} and~\ref{line:ra_sched2} specify
scheduling primitives in Listing~\ref{code:treernn_ra}. We propose the
following scheduling primitives to exploit these opportunities:

\begin{figure*}% >>>
  \centering
  \begin{minipage}[t]{.45\linewidth}
    \subcaptionbox{Recursive refactoring\label{fig:rec_refactoring}}
      {\includegraphics[width=\linewidth]{fig/hoisting.pdf}}%
  \end{minipage}%
  \hfill
  \begin{minipage}[b]{.45\linewidth}
    \subcaptionbox{Execution with and without dynamic batching. Numbers
     indicate node processing order. Nodes with the same number can
     be processed in parallel. Colors are added for emphasis.\label{fig:dyn_batch}}
      {\includegraphics[width=1\linewidth]{fig/dynamic_batching}}
    \subcaptionbox{Unrolling\label{fig:unrolling}}
      {\includegraphics[width=1\linewidth]{fig/unrolling}}%
  \end{minipage}%
  \caption
    {%
      Recursive scheduling primitives.%
      \label{fig:rec_sched}%
    }%
\end{figure*}% <<<

\noindent\textbf{Dynamic Batching: } Past work~\cite{dynet2,
  cell_batch, tffold, cavs} has proposed batching operators on-the-fly
in models with dynamic control flow to exploit parallelism in a
batch. This is referred to as dynamic batching. Since all control flow
in the models we look at depends only on the input data structure
(property~\ref{prop:ds_ctrl}), we perform dynamic batching in the data
structure linearizer. As in Cavs, we perform dynamic batching over
data structure nodes, as opposed to individual tensor operators. The
execution ordering of nodes of a tree with and without dynamic
batching is illustrated in Fig.~\ref{fig:dyn_batch}.

%% \begin{figure}
%%   \centering
%%   \includegraphics[width=0.80\linewidth]{fig/dynamic_batching}
%%   \caption{Execution with and without dynamic batching. The numbers
%%     indicate the node processing order. Nodes with the same number can
%%     be processed in parallel. Colors are added for more emphasis.}
%%   \label{fig:dyn_batch}
%% \end{figure}

\noindent\textbf{Specialization: } Recursive computations tend to have
frequent conditional checks to check for the base condition. The
overhead of such checks can be reduced if we amortize the check over
multiple nodes during execution. For example, we can process the
leaves and internal nodes of a data structure
separately. Specialization also opens opportunities for computation
hoisting (described in \S\ref{sec:comp_hoisting}). Note how the
generated ILIR in Listing~\ref{code:treernn_ilir} has separate loop
nests for the computation of leaves and internal nodes as the user
provided the specialization primitive for the base case condition on
line~\ref{line:ra_sched1} in Listing~\ref{code:treernn_ra}.

\noindent\textbf{Unrolling: } Unrolling recursion changes the order in
which the nodes are processed (as illustrated in
Fig~\ref{fig:unrolling}), moving the children's computatations closer
in time to their parent's computation. This allows reuse of the
children's hidden state via fast on-chip caches, as opposed to the
slower off-chip memories. Unrolling also opens up more opportunities
for kernel fusion. For example, we can fuse operators corresponding to
the children's computations after unrolling.


%% \noindent\textbf{Unrolling: } Unrolling recursion can allow us to
%% exploit data reuse across a node's computation and that of its
%% children. It changes the order in which the nodes are processed (as
%% illustrated in Fig~\ref{fig:unrolling}), moving the children's
%% computatations closer in time to their parent's computation. This
%% allows reuse of the children's hidden state via small, but fast
%% on-chip caches, as opposed to the slower off-chip
%% memories. \ppf{Mention increased batching opportunities}.

%% \begin{figure}
%%   \centering \includegraphics[width=0.80\linewidth]{fig/unrolling}
%%   \caption{Change in execution schedule due to unrolling}
%%   \label{fig:unrolling}
%% \end{figure}

\noindent\textbf{Recursive Refactoring: } Kernel fusion is harder to
perform across recursive call boundaries. In such cases, recursive
refactoring can be used to change the recursive backedge to make such
optimizations easier. This involves specifying a new backedge in the
form of a cut across the computation graph that makes up the body of
the recursive computation.

Consider the computation before refactoring is performed in
Fig.~\ref{fig:rec_refactoring}. \verb+A1+, \verb+A2+ and \verb+B+
represent tensor programs such that there is a dependence from
\verb+A1+ to \verb+A2+. In this case, the recursive backedge goes from
\verb+B+/\verb+A2+ to \verb+A1+. Fusing kernels in \verb+A1(n)+ and
\verb+A2(n.left)+ or \verb+A2(n.right)+ would be hard as the kernels
lie across a recursive call boundary. Instead, after refactoring, we
change the boundaries of recursive calls (the recursive backedge now
goes from \verb+A1+ to \verb+A2+) and thus \verb+A1(n)+,
\verb+A2(n.left)+ and \verb+A2(n.right)+ now lie in the same call and
can easily be fused.

%% \begin{figure}
%%   \centering
%%   \includegraphics[width=0.80\linewidth]{fig/hoisting}
%%   \caption{Recursive refactoring changes recursion backedge}
%%   \label{fig:rec_refactoring}
%% \end{figure}


Note that the unrolling and recursive refactoring transforms can lead
to repeated and redundant computations in the case of DAGs as a node
can have multiple parents. As a result, we do not support this case.

\subsection{Data Structure Linearizer}\label{sec:ds_linearizer}
The data structure linearizer traverses the input pointer linked
structure and lays it out in the form of arrays for the lowered
loop-based computation to iterate upon. The code for the data
structure linearizer is generated during the recursive lowering
pass. The pseudocode for the data structure linearizer for our running
example is shown below.

\begin{minted}[escapeinside=||,linenos,numbersep=4pt,frame=lines,fontsize=\scriptsize]{python}
leaf_batch, internal_batches = [], [[]]
left, right = [], []

def linearizer(n):
  if isleaf(n): leaf_batch.add(node)
  else:
    linearizer(n.left)
    linearizer(n.right)
    left[n], right[n] = n.left, n.right
    internal_batches[node.height].add(node)

leaf_batch_size = len(leaf_batch)
batch_sizes = [len(b) for b in internal_batches]
num_internal_batches = len(internal_batches)
num_batches = num_internal_batches + 1
\end{minted}

\subsection{Irregular Loops IR (ILIR)}\label{sec:ilir_api}
The recursive computation in RA, which involves data structure
accesses, when lowered to ILIR gives rise to indirect memory accesses
as well as loops with variable loop bounds. This can be seen in
Listing~\ref{code:treernn_ilir} which shows the generated ILIR for our
simple example model. Note how the variable \verb+node+ used to index
the tensor \verb+rnn+ in the loop on line~\ref{line:loop1} is a
non-affine function of the loop variable \verb+n_idx+. Furthermore,
the loop on line~\ref{line:loop4}, which iterates over a batch of
nodes has a variable bound, as batches can be of different lengths.


%% \begin{listing}[h]
%% \begin{minted}[escapeinside=||,linenos,numbersep=4pt,frame=lines,fontsize=\scriptsize]{python}
%% # rnn[node_dim, hidden_dim]
%% for n_idx in range(leaf_batch_size):      # batch_dim
%%   node = leaf_batch[n_idx]                                             |\label{line:node_load1}|
%%   for i in range(256):                    # hidden_dim
%%     rnn[node,i] = h0[i]

%% for b_idx in range(num_internal_batches): # all_batches_dim
%%   for n_idx in range(batch_sizes[b_idx]): # batch_dim
%%     node = internal_batches[b_idx,n_idx]                               |\label{line:node_load2}|
%%     for i in range(256):                  # hidden_dim
%%       rnn[node,i] = rnn[left[node],i] +
%%         rnn[right[node],i]
%% \end{minted}
%% \captionof{listing}{Named dimensions}
%% \label{code:named_dims}
%% \end{listing}


\begin{listing}[h]
\begin{minted}[escapeinside=||,linenos,numbersep=4pt,frame=lines,fontsize=\scriptsize]{python}
# rnn[node_dim, hidden_dim]
for n_idx = 0:leaf_batch_size:           # batch_dim                   |\label{line:loop1}|
  node = leaf_batch[n_idx]                                             |\label{line:node_load1}|
  for i = 0:256:                         # hidden_dim
    rnn[node,i] = Emb[word[node],i]

for b_idx = 0:num_internal_batches:      # all_batches_dim
  for n_idx = 0:batch_sizes[b_idx]:      # batch_dim                   |\label{line:loop4}|
    node = internal_batches[b_idx,n_idx]                               |\label{line:node_load2}|
    for i = 0:256:                       # hidden_dim
      lh[node,i] = rnn[left[node],i]
    for i = 0:256:                       # hidden_dim
      rh[node,i] = rnn[right[node],i]
    for i = 0:256:                       # hidden_dim
      rnn[node,i] = tanh(lh[node,i] + rh[node,i])
\end{minted}
\captionof{listing}{ILIR generated for the model in
  Fig.~\ref{fig:treelstm}}
\label{code:treernn_ilir}
\end{listing}

We therefore must extend the tensor compiler, as described in
\S\ref{sec:tensor_comp}, to support (1) non-affine index expressions,
(2) loops with variable bounds, and (3) conditional operators.

\subsubsection{Tensor Data Layouts}
Data layouts of intermediate tensors often need to be changed to allow
for an efficient use of the memory subsystem. This can involve
ensuring non-conflicting accesses to the GPU shared memory, or
sequential accesses to memory on a CPU and so on. To facilitate such
optimizations, the ILIR exposes data layout primitives, which allow
tensor dimensions to be split, reordered and fused, similar to the
corresponding loop transformations.

In accelerators with manually managed scratchpad memories such as a
GPU, optimizations such as tiling or kernel fusion require explicitly
caching parts of tensors in the scratchpad. This is not
straightforward for tensors indexed with non-affine index
expressions. Indexing the cached copy of a tensor with non-affine
index expressions would lead to a sparsely filled cache tensor, as the
indexing space is not generally contiguous. Such a sparsely filled
cached copy would occupy more memory than needed, which is problematic
as scratchpad memory space is often at a premium. Here, we exploit the
fact that in our case the non-affine index expressions correspond to
data structure accesses. As the data structure linearizer ensures that
we only process a data structure node once, there exists a one-to-one
relationship between index expression and the loop induction
variables. We can therefore index cached tensors by the contiguous
loop iteration space instead. This transformation also reduces
indexing costs by turning indirect memory accesses into affine
accesses. We expose this transformation as a scheduling primitive as
well.

%% \ppf{This paragraph seems out of place here. Move this somewhere
%%   else.} The ILIR is similar to the API of a tensor
%% compiler. Specifically, it provides all the common scheduling
%% primitives that a tensor compiler provides, which can be used to
%% further schedule the loop-based computation. While it can be difficult
%% to manually scheduled this lowered form of the recursive computation,
%% we note that there has been significant past work~\cite{halide_auto1,
%%   halide_auto2, tvm_autotune, tvm_autosched} in the field of
%% auto-scheduling which can be used here in a straightforward manner.

\subsubsection{Named Dimensions}\label{sec:named_dims}
\ppf{This section is too long.} In a tensor compiler, generally, there
is a one-to-one correspondence between the dimensions of a tensor and
the loop nest generated for its corresponding operator\footnote{We do
not cover the case of optimizations such as loop splitting which give
rise to additional loops here for brevity. Similarly, operators
involving reduction are not covered here.}. This can be seen in
Fig.~\ref{fig:tensor_comp_eg}, where two loops, each corresponding to
a dimension of the tensor \verb+r+ are generated (shown in the
generated code on the right). This one-to-one correspondence does not
hold for our case, as is apparent in the ILIR in
Listing~\ref{code:treernn_ilir}. Tensors \verb+lh+, \verb+rh+ and
\verb+rnn+ have two dimensions each, but the generated ILIR has three
loops for each of their corresponding operators. The relationship
between the tensor dimensions and the loop nests is used in the bounds
inference pass (described in \S\ref{sec:bounds}) as part of lowering.

In order to adapt the bounds inference pass for our case (as described
in \S\ref{sec:bounds}), we require the relationship to be explicitly
specified in the ILIR by the way of \emph{named dimensions}. Named
dimensions are identifiers associated with tensor dimensions and
loops, which allow us to explicitly specify and keep track of the
relationships between loops and tensor dimensions.





%% \ppf{This section looks too long.} Generally, in a tensor compiler,
%% there is a one-to-one correspondence between the loops generated when
%% lowering an operator and the dimensions of the tensor it
%% produces \footnote{We do not cover the case of optimizations such as
%% loop splitting which give rise to additional loops here for
%% brevity. Similarly, operators involving reduction are not covered
%% here.}. Note how the operator \verb+r+ in
%% Fig.~\ref{fig:tensor_comp_eg} produces a tensor of two dimensions,
%% each of which corresponds to a loop in the generated IR (shown on the
%% right side of the figure). This correspondence plays an important part
%% in the bounds inference pass during lowering, which we describe in
%% further detail in \S\ref{sec:bounds}.

%% This one-to-one correspondence does not hold for our case, as is
%% apparent in the ILIR in Listing~\ref{code:treernn_ilir}. Tensors
%% \verb+lh+, \verb+rh+ and \verb+rnn+ have two dimensions each, but the
%% generated ILIR has three loops for each of their corresponding
%% operators. We therefore require the ILIR to specify the relationship
%% explicitly by the way of \emph{named dimensions}. Named dimensions are
%% identifiers associated with tensor dimensions and loops, which allow
%% us to explicitly specify and keep track of the relationships between
%% tensor dimensions and the loops in an operator's loop nest. We discuss
%% the need for this explicit relationship in \S\ref{sec:bounds}.

Consider the ILIR in Listing~\ref{code:treernn_ilir} which shows
the named dimensions annotated as comments. The dimensions of the
tensor \verb+rnn+ are labeled with the named dimensions
\verb+node_dim+ and \verb+hidden_dim+. The tensor index dimension
\verb+node_dim+ corresponds to the two loop dimensions
\verb+all_batches_dim+ and \verb+batch_dim+.

%% In the case of \verb+node_dim+ as the relationship is non-affine
%% (consisting of the memory load on lines~\ref{line:node_load1}
%% and~\ref{line:node_load2}), we use uninterpreted functions to
%% represent it as discussed in \S\ref{sec:uninterp_fun}.


Named dimensions also make the semantic meaning of loops and index
expressions explicit. For example, the first dimension of the tensor
\verb+rnn+ is labelled \verb+node_dim+ and corresponds to the space of
all nodes. It, therefore, does not make sense to index \verb+rnn+ by
\verb+b_idx+, the loop variable for the loop associated with
\verb+all_batches_dim+.







%% Named dimensions also make the semantic meaning of loops and index
%% expressions explicit. For example, the loops corresponding to the
%% dimensions \verb+all_batches_dim+ and \verb+batch_dim+ iterate over
%% two semantically different entities --- all batches and the nodes in a
%% particular batch. The tensor \verb+rnn+ is indexed by \verb+node_dim+
%% in its first dimension. It does not make sense, for example, to index
%% \verb+rnn+ by \verb+b_idx+, or \verb+n_idx+, as they do not correspond
%% to data structure nodes.

\subsection{Lowering RA to ILIR}\label{sec:rec_lower}
We now discuss how \Sys~lowers the input RA computation to ILIR and
the data structure linearizer. The input computation may contain some
scheduling primitives as we saw in \S\ref{sec:rec_sched}. The
transformations of unrolling and recursive refactoring, if requested
by the user, are applied to the RA computation first. Branches that
need to be specialized and dynamic batching are both handled later
during the ILIR and linearizer generation stages as described below.

\subsubsection{Data Structure Linearizer Generation}
In the absence of specialization and dynamic batching, the linearizer
essentially has to traverse the data structure as the input program
does, while keeping track of the order of nodes encountered. This
ordering over the nodes would satisfy data dependences and can be used
during the tensor computations. As a result, in this simple case, the
data structure linearizer is essentially the input program, stripped
of all tensor computation. For conditional checks marked for
specialization, the linearizer has to separately collect nodes that
follow each of the two branches of the check. If dynamic batching is
desired, we would have to emit code to traverse the data structure and
identify batches of nodes that can be processed in parallel.


%% We now discuss how each of the scheduling primitives affect the
%% linearizer. Note that unrolling and recursive refactoring are already
%% handled at this stage as described above.

%% \noindent\textbf{Specialization: } For each conditional check marked
%% for specialization, the linearizer has to separately collect nodes
%% that follow each of the two branches of the check.

%% \noindent\textbf{Dynamic Batching: } If the user wishes to dynamically
%% batch the computation, instead of generating a total order over the
%% nodes of the data structure, the linearizer generates batches of nodes
%% across all input data structures, each of which can be processed in
%% parallel.

\subsubsection{ILIR Generation}\label{sec:ilir_gen}
When lowering the recursive RA computation to the loop-based ILIR, we
need to make temporary tensors explicit. Note, for example, in the
ILIR in Listing~\ref{code:treernn_ilir}, the tensors \verb+lh+ and
\verb+rh+ are explicitly created. We also materialize the tensor
\verb+rnn+, which stores the result of the computation. Each of the
tensors \verb+lh+, \verb+rh+ and \verb+rnn+ store data for each
recursive call, which in this case amounts to each tree node.


%% The lowering from RA to ILIR is, in essence, a lowering from recursion
%% to iteration. Just as we need to make the stack explicit in such a
%% lowering in general purpose programs, we need to make explicit all the
%% temporary tensors when lowering to ILIR. Note, for example, in the
%% ILIR in Listing~\ref{code:treernn_ilir}, the tensors \verb+lh+ and
%% \verb+rh+ are explicitly created. We also materialize the tensor
%% \verb+rnn+, which stores the result of the computation. Each of the
%% tensors \verb+lh+, \verb+rh+ and \verb+rnn+ store data for each
%% recursive call, which in this case amounts to each tree node.

As noted above, the scheduling primitives of unrolling and recursive
refactoring are already handled by the time we get to the lowering
stage. Specialized branches are handled by generating two versions of
the computation, each specialized for one target of the branch. The
data structure linearizer partitions nodes for such specialized
branches and the ILIR appropriately executes the correct version of
the computation for the each of the node partitions.

Depending on whether the user wishes to perform dynamic batching, the
lowering phase generates the appropriate loops that iterate over the
output of the data structure linearizer. Thus, if the user performs
dynamic batching, the ILIR would iterate over batches of nodes (as in
Listing~\ref{code:treernn_ilir}), while if they don't the code will
iterate over the nodes themselves.

\textbf{Memory Management and Dynamic Batching: } \ppf{This seems out
  of place.} When using dynamic batching with vendor libraries, one
needs to ensure that inputs to the batched kernel calls are contiguous
in memory. The resulting checks and memory copy operations have
significant overheads in past work~\cite{cavs}. As \Sys~does not rely
on vendor libraries, instead generating code for the entire program
itself, it is free from such memory layout restrictions.

%% While contiguous memory can be beneficial for kernel
%% performance, we find that the benefits of this approach outweigh the
%% overheads.

%% \subsubsection{Eager Computation Execution}
\subsubsection{Computation Hoisting and Constant Propagation}
\label{sec:comp_hoisting}
Recursive and iterative models often use an initial value for the base
case. If this initial value is same for all leaves for the data
structure the same computation is performed for all leaves. When
lowering to the ILIR, such computation is hoisted out of the recursion
to prevent redundant execution. We also specialially optimize for the
case when the initial value is the zero tensor.

\subsection{Irregular Loops IR to Hardware Code}\label{sec:ilir_lower}
As we saw in \S\ref{sec:ilir_api}, the ILIR extends a tensor compiler
with indirect indexing, conditional operators and variable loop
bounds. In this section, we describe the modifications to the
mechanism of a tensor compiler to support these extensions.

\subsubsection{Indirect Memory Accesses}\label{sec:uninterp_fun}
The ILIR allows indirect memory accesses. We represent the non-affine
index expressions arising as part of indirect memory accesses as
uninterpreted functions of loop variables. Analysis passes involving
such indirect memory accesses therefore perform symbolic analysis on
such uninterpreted functions. We use the Z3 SMT solver~\cite{z3} for
this purpose.


\subsubsection{Bounds Inference}
\label{sec:bounds}
As part of code generation, a tensor compiler infers loop bounds for
all operators in the input program in the bounds inference pass. The
pass processes the operator DAG starting from the output operators. As
a result, when an operator is being processed, the loop bounds of all
the loops of its consumers have been already inferred. For an operator
$op$, producing a tensor $t$, the pass iterates over all of its
consumers. For each dimension of $t$, each consumer computes how much
of $t$ it requires. The requirements of all consumers taken together
determine what parts of $t$ need to be computed. This quantity is then
translated to the loop bounds for $op$. The relationship between the
loops of an operator and the corresponding tensor dimensions becomes
important here. As we saw in \S\ref{sec:named_dims}, this relationship
is implicitly encoded in a traditional tensor compiler. In ILIR the
explicitly specified relationship via named dimensions is used
instead.


%% As part of code generation, a tensor compiler needs to infer loop
%% bounds for all operators in the input program. A simplified version of
%% this bounds inference pass is shown in Alg.~\ref{alg:bounds_infer}. In
%% the following text, we use the notation as described in the algorithm.

%% \begin{algorithm}
%%   \footnotesize
%%   \caption{Loop bounds inference in tensor compilers}
%%   \label{alg:bounds_infer}
%%   \hspace{\algorithmicindent} \textbf{Input:                           } \\
%%   \hspace{\algorithmicindent} $P$  \Comment{Input tensor program} \\
%%   \hspace{\algorithmicindent} $O$ \Comment{Set of all operators in $P$} \\
%%   \hspace{\algorithmicindent} $T$  \Comment{Set of all tensors in $P$} \\
%%   \hspace{\algorithmicindent} $T_f: O \rightarrow T$  \Comment{Operator to its produced tensor} \\
%%   \hspace{\algorithmicindent} $C: O \rightarrow 2^{O}$ \Comment{Operator to its consumers} \\
%%   \hspace{\algorithmicindent} $ND: T \rightarrow I$ \Comment{Tensor to number of its dimensions} \\
%%   \hspace{\algorithmicindent} $R = I \times I$ \Comment{The space of integer ranges} \\
%%   \hspace{\algorithmicindent} $B: Map<(O, I), R>$ \Comment{Loop bounds store} \\

%%   \vspace{0.1pt}

%%   \begin{algorithmic}[1]
%%     \Procedure{ComputeReqRange}{$t, i, c$}
%%     \State Given the bounds inferred for $c$, compute the required
%%       range of tensor $t$'s ith dimension
%%     \EndProcedure{}


%%     \Procedure{GetLoopBounds}{$op, Dom$}
%%     \EndProcedure{}


%%     \Procedure{InferBound}{}
%%     \For{\texttt{$op$ in $reverseTopSort(P)$}}
%%     \For{\texttt{$i$ in $0:ND(op)$}}
%%     \State $Dom \gets \emptyset$
%%     \For{\texttt{$c$ in $C(op)$}}                                            \label{line:c_for}
%%     \State $Dom_c \gets ComputeReqRange(T(op), i, c)$
%%     \State $Dom \gets Dom \cup Dom_c$
%%     \EndFor{}

%%     \State $B[(op, i)] \gets GetLoopBounds(op, Dom)$                          \label{line:translation}
%%     \EndFor{}
%%     \EndFor{}
%%     \EndProcedure{}
%%   \end{algorithmic}
%% \end{algorithm}


%% The bounds inference pass processes the operator DAG starting from the
%% output operators. As a result, when an operator is being processed,
%% the loop bounds of all the loops of its consumers have been already
%% inferred. For an operator $op$, producing a tensor $t = T_f(op)$, the
%% pass iterates over all of its consumers $C(op)$
%% (line~\ref{line:c_for}). For each dimension of $t$, each consumer $c$
%% computes how much of $t$ it requires in the function
%% \textsc{ComputeReqRange}. The requirements of all consumers taken
%% together tell us what parts of $t$ need to be computed. This quantity
%% is then translated to the loop bounds for $op$ in
%% line~\ref{line:translation}. The relationship between the loops of an
%% operator and the corresponding tensor dimensions becomes important
%% here. As we saw in \S\ref{sec:named_dims}, this relationship is
%% implicitly encoded in a traditional tensor compiler. In ILIR instead,
%% the explicitly specified relationship between tensor dimensions and
%% loop induction variables via the named dimensions is used.



\subsubsection{Caching Tensors}\label{sec:caching}
We discussed in \S\ref{sec:caching} how it is beneficial to index
cached copies of intermediate tensors by the dense loop iteration
space as opposed to the node space. A similar situation occurs when a
caching a tensor accessed by multiple non-affine index
expressions. Assume, for example, if we wished to cache the tensor
\verb+rnn+ in the \verb+ib+ loop nest in
Listing.~\ref{code:treernn_ilir}, for the purposes for the accesses
\verb+rnn[left[node],i]+ and \verb+rnn[right[node],i]+. We create a
cached tensor with an additional dimension corresponding to the
multiple non-affine index expressions, as shown in the listing below.

%% \begin{listing}[h]
\begin{minted}[escapeinside=||,linenos,numbersep=4pt,frame=lines,fontsize=\scriptsize]{python}
  for b_idx = 0:num_internal_batches:
    for n_idx = 0:batch_sizes[b_idx]:
      node = internal_batches[b_idx,n_idx]
      for i = 0:256:
        rnn_cache[b_idx,n_idx,i,0] = rnn[left[node],i]
        rnn_cache[b_idx,n_idx,i,1] = rnn[right[node],i]

  for b_idx = 0:num_internal_batches:
    for n_idx = 0:batch_sizes[b_idx]:
      node = internal_batches[b_idx,n_idx]
      for i = 0:256:
        rnn[node,i] = tanh(rnn_cache[b_idx,n_idx,i,0] +
                           rnn_cache[b_idx,n_idx,i,1])
\end{minted}
%% \captionof{listing}{Caching tensors indexed by non-affine index
%%   expressions}
%% \label{code:variant_cache}
%% \end{listing}

\subsubsection{Conditional Operator}\label{sec:cond_op}
To lower conditional checks such as the \verb+isleaf+ check in out
model, we add a conditional operator to the ILIR. This operator takes
two sub-graphs and a conditional check as an input. The conditional
operator lowers down to an \verb+if+ statement in the generated code.

%% The code that would be generated if we did not specialize the
%% condition in our running is shown below (\verb+lh+ and \verb+rh+
%% inlined for brevity).

%% %% \begin{listing}[h]
%%   \begin{minted}[escapeinside=||,linenos,numbersep=4pt,frame=lines,fontsize=\scriptsize]{python}
%% for b_idx = 0:num_batches:
%%   for n_idx = 0:batch_sizes[b_idx]:
%%     node = internal_batches[b_idx,n_idx]
%%     if (isleaf(node)):
%%       for i = 0:256:
%%         rnn[node,i] = Emb[word[n],i]
%%     else:
%%       for i = 0:256:
%%         rnn[node,i] = tanh(rnn[left[node],i] +
%%                            rnn[right[node],i])
%%   \end{minted}
%% %% \captionof{listing}{Conditional checks in lowered code}
%% %% \label{code:conditional}
%% %% \end{listing}


\subsection{Other Optimizations}\label{sec:other_opts}
Below, we discuss a few less important optimizations and scheduling
knobs we implemented.

\noindent\textbf{Loop Peeling: } The generated ILIR in \Sys~involves
loops with variable loop bounds. Splitting such loops gives rise to
bounds checks in the bodies of the loops. We employ loop peeling to
ensure that such checks are only employed for the last few iterations
of the loop.

\noindent\textbf{GPU Global Barriers: } \Sys~generated code often
contains cross-thread synchronization. For the GPU backend, we find
that the grid barrier implementation provided by the CUDA
API~\cite{grid_sync} requires a high number of registers. As GPU
registers are at a premium (especially as we persist the model in the
registers), this barrier implementation cannot always be employed. We
then fall back to the slower lock-based implementation proposed
in~\cite{barrier}.

\noindent\textbf{Rational Approximations of Nonlinear Functions: } We
use rational approximations for $tanh$ and $sigmoid$ which makes
exploiting SIMD instructions on CPUs easier.


==> src/discussion.tex <==
\section{Discussion}\label{sec:discuss}
Past work on machine learning compilers~\cite{relay, nimble,
  tf_ctrl_flow, tf_ctrl_flow_sched} as well as on designing
models~\cite{treelstm, moe, depth_adapt_transformer} suggests that
supporting efficient execution of various kinds of dynamism in ML
models is very desirable. We believe that \Sys~is an important
stepping stone in this direction. In developing techniques to support
such dynamism, based on our work with \Sys, we believe it is important
to exploit past work on general purpose compilation, such as partial
evaluation (as can be seen in the linearization step of \Sys), or the
sparse polyhedral framework. It is also important to expand the scope
of the highly specialized ML frameworks and techniques used today
(without compromising their ability to optimize static feed-forward
models), as we do in the case of the ILIR, for example.


==> src/linearization_table.tex <==
Batch Size & TreeLSTM/TreeGRU/MV-RNN & DAG-RNN & TreeFC \\ \hline
1 & 1.31 & 8.2 & 3.04 \\
10 & 9.64 & 95.14 & 30.36 \\

